Towards Interpretable Deep Metric Learning with Structural Matching

How do the neural networks distinguish two images? It is of critical importance to understand the matching mechanism of deep models for developing reliable intelligent systems for many risky visual applications such as surveillance and access control. However, most existing deep metric learning methods match the images by comparing feature vectors, which ignores the spatial structure of images and thus lacks interpretability. In this paper, we present a deep interpretable metric learning (DIML) method for more transparent embedding learning. Unlike conventional metric learning methods based on feature vector comparison, we propose a structural matching strategy that explicitly aligns the spatial embeddings by computing an optimal matching flow between feature maps of the two images. Our method enables deep models to learn metrics in a more human-friendly way, where the similarity of two images can be decomposed to several part-wise similarities and their contributions to the overall similarity. Our method is model-agnostic, which can be applied to off-the-shelf backbone networks and metric learning methods. We evaluate our method on three major benchmarks of deep metric learning including CUB200-2011, Cars196, and Stanford Online Products, and achieve substantial improvements over popular metric learning methods with better interpretability. Code is available at https://github.com/wl-zhao/DIML

==> tables/components.tex <==
\begin{table}[tbp]
  \centering
  \caption{\textbf{Effects of the three components in our \ours:} Structural Similarity (SS), Multi-scale Matching (MM) and Cross Correlation (CC). We show that our method can enhance the performance of the baseline methods by combining the three components together.}
  \adjustbox{max width=\linewidth}{
  \setlength{\tabcolsep}{2pt}
    \begin{tabu}to 1.45\linewidth{c*{3}{X[c]}*{6}{X[c]}}\toprule
    \multirow{2}[0]{*}{\textbf{Baseline}} & \multicolumn{3}{c}{\textbf{Components}} & \multicolumn{2}{c}{\textbf{CUB200-2011}} & \multicolumn{2}{c}{\textbf{Cars196}} & \multicolumn{2}{c}{\textbf{SOP}} \\\cmidrule(rl){2-4}\cmidrule(rl){5-6}\cmidrule(rl){7-8}\cmidrule(rl){9-10}
          & SS     & MM     & CC    & \textbf{P@1} &  \textbf{M@R} & \textbf{P@1} & \textbf{M@R} & \textbf{P@1}  & \textbf{M@R} \\\midrule
    \multirow{4}[0]{*}{Margin~\cite{wu2017sampling}} &       &       &       & 62.47   & 23.14  & 72.18    & 20.82  & 78.39   & 42.34  \\
          & \cmark &       &       & 63.64    & 22.52  & 74.86    & 21.24  & \textit{\ul{77.30}}  &  \textit{\ul{41.02}}  \\
          & \cmark & \cmark &       & 64.96    & 23.87  & 76.02    & 22.02  & 78.53    & 42.45  \\
          & \cmark & \cmark & \cmark & \textbf{65.16} & \textbf{24.51} & \textbf{76.62}  & \textbf{22.48} & \textbf{79.26} & \textbf{43.19} \\\midrule
    \multirow{4}[0]{*}{MS~\cite{wang2019multi}} &       &       &       & 62.56    & 21.99  & 74.81   & 21.60  & 77.90 & 41.54  \\
          & \cmark &       &       & 63.52   & 21.66  & 75.63    & 21.10  & \textit{\ul{75.81}}    & \textit{\ul{39.38}}  \\
          & \cmark & \cmark &       & 64.40    & 22.83  & 77.39   & 22.77  & 77.87   & 41.55  \\
          & \cmark & \cmark & \cmark & \textbf{64.89} & \textbf{23.34} & \textbf{78.44} & \textbf{23.31} & \textbf{78.53}  & \textbf{42.22} \\\bottomrule
    \end{tabu}%
    }
  \label{tab:ablation}%
\end{table}%

==> tables/embedding_size.tex <==
\begin{table}[tbp]
  \centering
\caption{\textbf{Effects of embedding size.} Our~\ours~is robust to the changing of the embedding size $D$ and can improve the performance of the baseline methods consistently.} \vspace{-5pt}
  \adjustbox{max width=\linewidth}{
    \begin{tabular}{clcccccc}\toprule
    \multirow{2}[0]{*}{$D$} & \multicolumn{1}{c}{\multirow{2}[0]{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{CUB200-2011}} & \multicolumn{3}{c}{\textbf{Cars196}} \\\cmidrule(lr){3-5}\cmidrule(lr){6-8}
          &       & \textbf{P@1} & \textbf{RP} & \textbf{M@R} & \textbf{P@1} & \textbf{RP} & \textbf{M@R} \\\midrule
    \multirow{6}[0]{*}{64} & Margin & 59.39  & 32.59  & 21.53  & 69.31  & 30.98  & 19.67  \\
          & Margin~\cite{wu2017sampling} + \ours & \textbf{62.98}  & \textbf{33.88}  & \textbf{22.95}  & \textbf{74.44}  & \textbf{31.96}  & \textbf{21.60}  \\\cmidrule{2-8}
          & MS~\cite{wang2019multi} & 58.52  & 31.35  & 20.23  & 71.67  & 30.90  & 19.57  \\
          & MS + \ours & \textbf{61.73}  & \textbf{32.61}  & \textbf{21.62}  & \textbf{76.94}  & \textbf{31.95}  & \textbf{21.72}  \\\cmidrule{2-8}
          & ProxyAnchor~\cite{kim2020proxy} & 62.56  & 34.61  & 23.45  & 78.08  & 34.35  & 23.95  \\
          & ProxyAnchor + \ours & \textbf{65.01}  & \textbf{35.53}  & \textbf{24.40}  & \textbf{83.11}  & \textbf{36.49}  & \textbf{26.55}  \\\midrule
    \multirow{6}[0]{*}{512} & Margin~\cite{wu2017sampling} & 64.92  & 35.94  & 24.92  & 73.68  & 32.03  & 21.09  \\
          & Margin + \ours & \textbf{66.91}  & \textbf{36.82}  & \textbf{25.89}  & \textbf{76.67}  & \textbf{32.62}  & \textbf{22.20}  \\\cmidrule{2-8}
          & MS~\cite{wang2019multi} & 65.92  & 35.14  & 24.17  & 76.85  & 33.93  & 22.78  \\
          & MS + \ours & \textbf{68.15}  & \textbf{36.04}  & \textbf{25.14}  & \textbf{79.74}  & \textbf{34.68}  & \textbf{24.01}  \\\cmidrule{2-8}
          & ProxyAnchor\cite{kim2020proxy} & 67.30  & 37.40  & 26.38  & 84.75  & 37.56  & 27.66  \\
          & ProxyAnchor + \ours & \textbf{67.93}  & \textbf{37.92}  & \textbf{26.88}  & \textbf{87.01}  & \textbf{39.03}  & \textbf{29.39}  \\\bottomrule
    \end{tabular}
    }
  \label{tab:embedding}%
\end{table}%

==> tables/fm_size.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{DIML/figs/ablation_G.pdf} \vspace{-5pt}
  \caption{\textbf{Effects of the size of feature map.} Generally, the performance of our \ours~is better with higher $G$. \ours~with $G=4$ yields good results within relatively low computational costs.}\label{fig:fm_size}
\end{figure}

==> tables/main_results.tex <==
\begin{table}[t]
  \centering
%   \small
% \midsepremove{}
  \caption{\textbf{Applying DIML to various deep metric learning methods.} Experimental results show that our method can improve the performance of all the methods consistently.} \vspace{-5pt}
 \adjustbox{max width=0.98\linewidth}{
 \setlength{\tabcolsep}{1pt}
    % \begin{tabular}{lccccccccc}\toprule
   \begin{tabu}to 1.45\linewidth{l*{3}{X[c]}|*{3}{X[c]}|*{3}{X[c]} } \toprule
    \multicolumn{1}{l}{\multirow{2}[0]{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{CUB200-2011}} & \multicolumn{3}{c}{\textbf{Cars196}} & \multicolumn{3}{c}{\textbf{SOP}} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
          & \multicolumn{1}{c}{\textbf{P@1}} & \textbf{RP} & \multicolumn{1}{c}{ \textbf{M@R}} & \textbf{P@1} & \textbf{RP} & \multicolumn{1}{c}{\textbf{M@R}} & \textbf{P@1} & \textbf{RP} & \textbf{M@R} \\\midrule


Contrasitive~\cite{hadsell2006dimensionality_contrastive} & 61.77 & 34.25 & 23.24 & 67.45 & 30.01 & 18.61 & 73.27 & 40.92 & 37.5 \\
+ \ours & \textbf{64.43} & \textbf{35.16} & \textbf{24.29} & \textbf{73.35} & \textbf{30.76} & \textbf{20.13} & \textbf{74.47} & \textbf{41.58} & \textbf{38.29} \\\midrule
Triplet-R~\cite{schroff2015facenet} & 58.34 & 32.00 & 20.93 & 62.73 & 26.95 & 15.24 & 66.60 & 33.62 & 30.26 \\
+ \ours & \textbf{60.60} & \textbf{32.63} & \textbf{21.74} & \textbf{67.92} & \textbf{27.65} & \textbf{16.72} & \textbf{68.73} & \textbf{35.04} & \textbf{31.79} \\\midrule
Triplet-S~\cite{schroff2015facenet} & 59.28 & 32.77 & 21.79 & 67.00 & 30.0 & 18.23 & 73.67 & 40.45 & 37.14 \\
+ \ours & \textbf{62.85} & \textbf{33.87} & \textbf{23.04} & \textbf{72.06} & \textbf{30.89} & \textbf{20.04} & \textbf{75.14} & \textbf{41.68} & \textbf{38.42} \\\midrule
Triplet-H~\cite{roth2020revisiting} & 61.39 & 33.21 & 22.15 & 71.76 & 32.53 & 20.83 & 73.28 & 39.98 & 36.56 \\
+ \ours & \textbf{62.02} & \textbf{33.50} & \textbf{22.49} & \textbf{74.75} & \textbf{32.94} & \textbf{21.76} & \textbf{73.62} & \textbf{40.14} & \textbf{36.79} \\\midrule
Triplet-D ~\cite{wu2017sampling} & 61.99 & 33.92 & 22.90 & 73.07 & 32.18 & 20.81 & 77.34 & 44.25 & 40.80 \\
+ \ours & \textbf{63.40} & \textbf{34.49} & \textbf{23.59} & \textbf{77.31} & \textbf{33.05} & \textbf{22.61} & \textbf{77.81} & \textbf{44.82} & \textbf{41.39} \\\midrule
NPair~\cite{sohn2016improved_npair} & 60.30 & 33.53 & 22.27 & 69.52 & 32.24 & 20.25 & 76.47 & 43.48 & 39.94 \\
+ \ours & \textbf{62.17} & \textbf{34.02} & \textbf{22.85} & \textbf{74.65} & \textbf{32.91} & \textbf{21.67} & \textbf{76.86} & \textbf{43.87} & \textbf{40.38} \\\midrule
Angular~\cite{wang2017deep} & 61.36 & 34.17 & 23.00 & 70.93 & 32.97 & 21.31 & 73.79 & 41.42 & 37.90 \\
+ \ours & \textbf{63.77} & \textbf{35.09} & \textbf{24.06} & \textbf{74.72} & \textbf{33.80} & \textbf{22.83} & \textbf{74.91} & \textbf{42.17} & \textbf{38.73} \\\midrule
GenLifted~\cite{hermans2017defense_genlift} & 58.27 & 32.86 & 21.83 & 66.88 & 30.96 & 19.00 & 74.84 & 42.28 & 38.66 \\
+ \ours & \textbf{61.07} & \textbf{33.82} & \textbf{22.98} & \textbf{72.95} & \textbf{31.93} & \textbf{20.88} & \textbf{75.92} & \textbf{43.08} & \textbf{39.55} \\\midrule
ProxyNCA~\cite{movshovitz2017no_pnca} & 62.76 & 35.05 & 24.03 & 71.05 & 31.62 & 20.55 & 74.70 & 41.32 & 37.96 \\
+ \ours & \textbf{64.75} & \textbf{36.02} & \textbf{25.10} & \textbf{74.86} & \textbf{32.43} & \textbf{22.00} & \textbf{76.17} & \textbf{42.65} & \textbf{39.36} \\\midrule
Histogram~\cite{evgeniya2016histogram} & 59.96 & 33.07 & 22.15 & 69.49 & 31.62 & 19.76 & 71.15 & 38.06 & 34.70 \\
 + \ours & \textbf{62.69} & \textbf{33.80} & \textbf{23.00} & \textbf{74.50} & \textbf{32.36} & \textbf{21.26} & \textbf{72.06} & \textbf{38.57} & \textbf{35.30} \\\midrule
Quadruplet~\cite{chen2017beyond_quadruplet} & 61.53 & 34.05 & 22.93 & 69.64 & 31.40 & 19.67 & 77.02 & 44.27 & 40.88 \\
+ \ours & \textbf{62.80} & \textbf{34.65} & \textbf{23.62} & \textbf{75.66} & \textbf{32.35} & \textbf{21.69} & \textbf{78.08} & \textbf{45.16} & \textbf{41.79} \\\midrule
SNR~\cite{yuan2019SNR} & 62.00 & 34.72 & 23.59 & 72.95 & 32.72 & 21.28 & 77.82 & 44.98 & 41.51 \\
+ \ours & \textbf{64.55} & \textbf{35.25} & \textbf{24.27} & \textbf{77.57} & \textbf{33.54} & \textbf{23.02} & \textbf{78.50} & \textbf{45.65} & \textbf{42.24} \\\midrule
%SoftTriplet~\cite{qian2019softtriple} & 61.21 & 32.83 & 22.29 & 68.95 & 30.71 & 19.43 & 52.12 & 21.98 & 19.41 \\
%SoftTriplet + \ours & \textbf{63.59} & \textbf{33.87} & \textbf{23.43} & \textbf{73.15} & \textbf{31.48} & \textbf{20.89} & \textbf{54.65} & \textbf{23.40} & \textbf{20.82} \\\midrule
Softmax~\cite{zhai2019classification_softmax} & 61.06 & 32.7 & 21.55 & 72.61 & 31.17 & 19.88 & 77.02 & 43.47 & 40.25 \\
+ \ours & \textbf{63.30} & \textbf{33.71} & \textbf{22.64} & \textbf{76.39} & \textbf{32.06} & \textbf{21.49} & \textbf{78.17} & \textbf{44.62} & \textbf{41.43} \\\midrule
%Triplet (Random)~\cite{schroff2015facenet} & 58.34 & 32.0 & 20.93 & 62.73 & 26.95 & 15.24 & 66.6 & 33.62 & 30.26 \\
% Triplet (Random) + \ours & \textbf{60.60} & \textbf{32.63} & \textbf{21.74} & \textbf{67.92} & \textbf{27.65} & \textbf{16.72} & \textbf{68.73} & \textbf{35.04} & \textbf{31.79} \\\midrule

Margin~\cite{wu2017sampling} & 62.47 & 34.12 & 23.14 & 72.18 & 32.00 & 20.82 & 78.39 & 45.64 & 42.34 \\ % beta 12
+ \ours & \textbf{65.16} & \textbf{35.37} & \textbf{24.51} & \textbf{76.62} & \textbf{32.85} & \textbf{22.48} & \textbf{79.26} & \textbf{46.44} & \textbf{43.19} \\\midrule
% Margin b06~\cite{wu2017sampling} & 62.27 & 34.98 & 23.87 & 70.97 & 32.02 & 20.54 & 77.23 & 44.8 & 41.46 \\
% Margin b06 + \ours & \textbf{64.70} & \textbf{35.66} & \textbf{24.72} & \textbf{75.45} & \textbf{32.79} & \textbf{22.13} & \textbf{78.18} & \textbf{45.48} & \textbf{42.19} \\\midrule
Arcface~\cite{deng2019arcface} & 61.39 & 33.70 & 22.4 & 73.37 & 31.90 & 20.52 & 77.55 & 44.44 & 41.07 \\
+ \ours & \textbf{64.72} & \textbf{34.88} & \textbf{23.72} & \textbf{77.24} & \textbf{32.88} & \textbf{22.34} & \textbf{78.52} & \textbf{45.45} & \textbf{42.10} \\\midrule
MS~\cite{wang2019multi} & 62.56 & 32.74 & 21.99 & 74.81 & 32.72 & 21.60 & 77.90 & 44.97 & 41.54 \\
+ \ours & \textbf{64.89} & \textbf{33.99} & \textbf{23.34} & \textbf{78.44} & \textbf{33.57} & \textbf{23.31} & \textbf{78.53} & \textbf{45.59} & \textbf{42.22} \\\midrule
ProxyAnchor~\cite{kim2020proxy} & 65.24 & 35.81 & 24.87 & 82.36 & 36.00 & 25.85 & 79.10 & 46.31 & 42.91 \\
+ \ours & \textbf{66.46} & \textbf{36.49} & \textbf{25.58} & \textbf{86.13} & \textbf{37.90} & \textbf{28.11} & \textbf{79.22} & \textbf{46.43} & \textbf{43.04} \\\bottomrule
% Average Improvement & 2.25 & 0.83 & 0.95 & 4.53 & 0.86 & 1.64 & 1.03 & 0.8 & 0.85 \\\bottomrule
    \end{tabu}
} \vspace{-10pt}
  \label{tab:main}
\end{table}

==> tables/training.tex <==
\begin{table}[tbp]
  \centering
  \caption{\textbf{Effects of training.} Our method can substantially improve the baseline model with or without training.}
  \label{tab:training}% 
  \vspace{-5pt}
  \adjustbox{max width=\linewidth}{
    \begin{tabular}{crccccccc}\toprule
    \multirow{2}[0]{*}{\textbf{Baseline}} & \multicolumn{2}{c}{\textbf{Setting}} & \multicolumn{2}{c}{\textbf{CUB200-2011}} & \multicolumn{2}{c}{\textbf{Cars196}} & \multicolumn{2}{c}{\textbf{SOP}} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
          & \multicolumn{1}{l}{\textbf{test}} & \multicolumn{1}{l}{\textbf{train}} & \textbf{P@1}  & \textbf{M@R} & \textbf{P@1}  & \textbf{M@R} & \textbf{P@1}  & \textbf{M@R} \\\midrule
    \multirow{3}[0]{*}{Margin~\cite{wu2017sampling}} &       &       & 62.47  & 23.14  & 72.18   & 20.82  & 78.39   & 42.34  \\
          & \cmark     &       & 65.16   & 24.54  & \textbf{76.65}   & \textbf{22.95}  & \textbf{79.26}    & \textbf{43.19}  \\
          & \cmark     & \cmark     & \textbf{65.36}    & \textbf{24.90}  & 75.61    & 22.34  & 78.81    & 42.89  \\\midrule
    \multirow{3}[0]{*}{MS~\cite{wang2019multi}} &       &       & 62.56    & 21.99  & 74.81    & 21.60  & 77.90    & 41.54  \\
          & \cmark     &       & 64.89  & 23.38  & 78.50    & \textbf{23.81}  & 78.53   & 42.23  \\
          & \cmark     & \cmark     & \textbf{65.72}  & \textbf{24.37}  & \textbf{78.90}    & 23.80  & \textbf{79.00}   & \textbf{42.96}  \\\bottomrule
    \end{tabular}%
    }
\end{table}%

==> tables/truncation_number.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{DIML/figs/ablation_K.pdf}
  \caption{\textbf{Comparisons of different truncation number.} We test for different truncation number $K$ ranging from 0 to 500. Experimental results show that a small $K$ can already bring considerable performance improvement.}
    \label{fig:truncation_number}
\end{figure}
